GaussianPretrain: A Simple Unified 3D Gaussian Representation for Visual Pre-training in Autonomous Driving

Self-supervised learning has made substantial strides in image processing, while visual pre-training for autonomous driving is still in its infancy. Existing methods often focus on learning geometric scene information while neglecting texture or treating both aspects separately, hindering comprehensive scene understanding. In this context, we are excited to introduce GaussianPretrain, a novel pre-training paradigm that achieves a holistic understanding of the scene by uniformly integrating geometric and texture representations. Conceptualizing 3D Gaussian anchors as volumetric LiDAR points, our method learns a deepened understanding of scenes to enhance pre-training performance with detailed spatial structure and texture, achieving that 40.6% faster than NeRF-based method UniPAD with 70% GPU memory only. We demonstrate the effectiveness of GaussianPretrain across multiple 3D perception tasks, showing significant performance improvements, such as a 7.05% increase in NDS for 3D object detection, boosts mAP by 1.9% in HD map construction and 0.8% improvement on Occupancy prediction. These significant gains highlight GaussianPretrain's theoretical innovation and strong practical potential, promoting visual pre-training development for autonomous driving. Source code will be available at https://github.com/Public-BOTs/GaussianPretrain

==> sec/1.1_intro_related.tex <==
% \vspace{-1em}
\section{Introduction}
\label{sec:intro}
With the development of autonomous driving technology, vision-centered solutions have gradually attracted widespread attention. Many studies focus on extracting bird's-eye view (BEV) features from multi-view input images to address various downstream applications. While supervised methods dominate current research, their reliance on accurate ground truth labels presents a significant bottleneck due to the high cost and difficulty of acquisition. Conversely, the abundance and accessibility of unlabeled data offer a promising avenue for improving performance. However, effectively harnessing this unlabeled data remains a significant and ongoing challenge in the field.

The core idea of self-supervised pre-training technology is to learn meaningful representations from abundant unlabeled data by leveraging carefully designed proxy tasks. There are several approaches have been developed to explore this topic in the field of autonomous driving. Methods like UniScene~\cite{min2023uniscene} and  ViDAR~\cite{yang2024visual} focus on predicting 3D occupancy or future LiDAR point clouds, effectively capturing geometric information but neglecting texture. Conversely,
%-------------
% Self-Occ~\cite{huang2024selfocc} and UniPAD~\cite{yang2024unipad} reconstruct 3D surfaces and RGB pixels from image-LiDAR pairs, learning texture but relying solely on depth maps for geometry, which aids in learning texture information. However, they are limited as they rely solely on depth maps for geometric information extraction. 
%---------------
Self-Occ~\cite{huang2024selfocc} and UniPAD~\cite{yang2024unipad} reconstruct 3D surfaces and RGB pixels from image-LiDAR pairs, thus capturing texture but relying solely on depth maps for geometric insights. Although this aids in texture learning, these methods remain limited in extracting comprehensive geometric information.
%------------------
OccFeat~\cite{sirko2024occfeat}, combines feature distillation with occupancy prediction to effectively capture both texture and geometry, but it introduces the complexity of an additional image foundation model and incurs significant pre-training costs.
%-------------------------------------------------------------------------

% Motivated by the success of 3D Gaussian Splatting in reconstruction benchmarks and MAE in 2D image self-supervised tasks, we propose a novel pre-training approach GaussianPretrain, which combines 3D Gaussian Splatting and MAE and extends it to 3D visual tasks. Specifically, we use masked multi-view images as input and then construct a 3D voxel using any view transformer method. Next, we use a set of Gaussian anchors in 3D space to learn Gaussian properties from the 3D voxel, simultaneously understanding the scene through 3D Gaussian Splatting of geometry and texture information. Unlike methods that use NeRF, such as UniPAD, we employ 3D Gaussian Splatting, which has lower training costs and memory consumption, to fully understand the geometry and texture information of the scene. By combining these advantages, our method can perform self-supervised pre-training effectively and cost-efficiently.
% The  3D Gaussian Splatting well addresses these issues,
%----------------- 
% Fortunately, 3D Gaussian Splatting (3D-GS) offers a powerful representation for scene reconstruction, encoding \textbf{geometric} and \textbf{texture} information through attributes like \textit{position, color, rotation, scaling, and opacity}.  All of these advantages address the key limitations of existing 3D pre-training techniques. Additionally, the training times of 3D-GS are on the order of minutes, enabling efficient learning and real-time rendering.
%--------------------

\shengyin{Fortunately, 3D Gaussian Splatting (3D-GS), structured as point clouds, offers a powerful representation for scene reconstruction, encoding \textbf{geometric} and \textbf{texture} information through attributes like \textit{position, color, rotation, scaling, and opacity}. Furthermore, compared to NeRF, 3D-GS achieves faster training convergence and requires less memory. All of these advantages address the key limitations in existing 3D pre-training techniques.}

% Additionally, the training times of 3D-GS are on the order of minutes, enabling real-time rendering and facilitating the reconstruction 

Inspired by the success of 3D-GS in various vision tasks and MAE~\cite{he2022masked} in 2D image self-supervised, we propose a novel pre-training approach \textbf{GaussianPretrain}, which combines 3D-GS with Ray-based MAE strategy for 3D visual tasks.  Our approach incorporates two key innovations: (i) \textbf{\textit{3D Gaussian anchor Guidance Strategy}}: We introduce a set of learnable  Gaussian anchors in 3D space to guide the learning of  Gaussian properties from the 3D voxel. This enables the model to simultaneously understand the geometry and texture information of the scene through 3D Gaussian Splatting. (ii). \textbf{\textit{Gaussian with Ray-based and MAE Strategy}}. To enhance the efficiency of our approach, we sample Gaussian points by launching a series of rays into 3D space and predict the related attributes (e.g., \textit{depth, opacity}) only for the valid masked patches. These patches are identified by an MAE strategy and further filtered to include only those with LiDAR depth supervision. Compared to 
NeRF~\cite{mildenhall2021nerf} based methods like UniPAD~\cite{yang2024unipad}, our GaussianPretrain offers lower training costs and memory consumption, while providing well understanding of the scene's representation. 
% In addition, the attributes of opacity are suitable for many 3D vision tasks, especially in occupancy.
By combining these advantages, our GaussianPretrain enables to perform effective and efficient self-supervised pre-training


\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/AAAI-top-0.pdf}
  \caption{
  Comparison of UVTR~\cite{li2022unifying} model performance on the nuScenes dataset with different pre-training framework: ImageNet, UniPAD~\cite{yang2024unipad}, and our GaussianPretrain.}
  \label{fig:top}
\end{figure}

% Specifically,we construct the 3D voxel space with any view transformer method,e.g.,\textcolor{red}{[cite]} which takes masked multi-view images as input. Next,

To demonstrate the effectiveness and generalizability of GaussianPretrain, we conduct extensive experiments on various downstream vision tasks using the large-scale nuScenes\cite{caesar2020nuscenes} dataset. 
%The results indicate that our method significantly outperforms existing supervised and unsupervised pre-training approaches. 
As shown in Figure~\ref{fig:top}, for 3D object detection, our pre-trained model significantly  achieves the 8.2\% mAP and 10\% NDS improvement compared to the baseline UVTR, pre-trained on ImageNet. Furthermore, our approach surpasses the previous state-of-the-art method, UniPAD~\cite{yang2024unipad}, by 0.5\% mAP and 1.05\% NDS. 
%This enhancement is attributed to our method's superior ability to capture geometric information. 
To further validate the generalizability, we evaluate our method on HD map construction and occupancy prediction tasks. GaussianPretrain surpasses the state-of-the-art method MapTR~\cite{liao2022maptr} method for HD map construction by 1.9\% in mAP For occupancy prediction, our approach achieves a 2.04\% improvement in mIoU over PanoOCC, setting a new state-of-the-art performance.
To summarize, our main contributions are as follows:
\begin{itemize}
    % \item To the best of our knowledge, we are the first to integrate 3D-GS technology into pre-training diagram, representing a novel contribution to this field. The GaussianPretrain, is a novel pre-training framework that integrates 3D geometric and texture information into a unified Gaussian representation, significantly advancing visual tasks for autonomous driving.
    %\item We proposed a simple unified Gaussian representation, By leveraging 3D Gaussian anchors as volumetric LiDAR points, employing the Ray-based and MAE strategy. our approach offers an innovative and efficient method for capturing detailed scene information, reducing computational and GPU memory costs while maintaining high fidelity.
    %\item GaussianPretrain demonstrates substantial improvements in multiple 3D perception tasks, e.g., 3D object detection, HD-Map segmentation, and Occupancy. Setting new performance standards and reinforcing its potential to revolutionize visual pre-training in autonomous driving.
    \item We introduce GaussianPretrain, a novel pre-training framework that integrates 3D Gaussian Splatting technology with a unified Gaussian representation. To the best of our knowledge, this is the first work to leverage 3D-GS for pre-training diagram, representing a novel contribution to this field.
    \item We propose a simple yet effective framework by leveraging 3D Gaussian anchors as volumetric LiDAR points, combined with Ray-based and Masked Autoencoder (MAE) strategy. Providing an efficient solution for high-fidelity scene capture, significantly reducing computational and GPU memory costs without sacrificing detail.
    \item The comprehensive experimental results of GaussianPretrain showcase significant improvements across various 3D perception tasks, including 3D object detection, HD-map segmentation, and Occupancy prediction. These advancements set new performance standards and underscore GaussianPretrain's transformative potential in visual pre-training tasks for autonomous driving applications.
\end{itemize}

\section{Related Work}
\subsection{Pre-training for Autonomous Driving.}
Pre-training in 2D images has achieved remarkable success, primarily through contrastive learning and masked signal modeling. These techniques focus on learning the semantic and texture information of images. However, pre-training for visual autonomous driving requires accurate geometrical representation, which presents additional challenges. Several works are currently exploring this area. For instance, UniScene\cite{min2023uniscene} and OccNet\cite{tong2023scene} leverage occupancy prediction for pre-training, while ViDAR~\cite{yang2024visual} predicts future LiDAR data from historical frame images. Although these methods are effective at capturing geometric information, but cannot learn detailed texture information. Conversely, approaches like Self-OCC\cite{huang2024selfocc}, UniPAD~\cite{yang2024unipad}, and MIM4D\cite{zou2024mim4d} utilize NeRF~\cite{mildenhall2021nerf} to render RGB images and depth maps, enabling them to learn texture while geometric information is insufficient. OccFeat\cite{sirko2024occfeat} employs knowledge distillation to transfer texture information from the image foundation model while performing occupancy prediction but incurs significant pre-training costs. Our work pioneers the use of 3D Gaussian Splatting for vision pre-training in autonomous driving. This innovative technique efficiently learns both texture and geometric information, overcoming the limitations of previous methods.


\subsection{3D Gaussian Splatting and NeRF.} 
Neural Radiance Fields (NeRF)~\cite{mildenhall2021nerf} achieve impressive rendering quality by implicitly representing scenes of color and density, parameterized by Multi-Layer Perceptrons (MLPs) combined with volume rendering techniques. Follow-up works \cite{boss2021nerd,park2021nerfies,wang2024perf,xian2021space,irshad2023neo} have extended NeRF to various tasks with promising results. However, these methods require time-consuming per-scene optimization, hindering their performance due to slow optimization and rendering speeds. In contrast, 3D Gaussian Splatting\cite{kerbl20233d} explicitly represents scenes using anisotropic Gaussians, enabling real-time rendering through differentiable rasterization. Nonetheless, Gaussian Splatting tends to overfit specific scenes, as it is heavily dependent on scene-specific optimization. To address this, recent approaches predict Gaussian parameters in a feed-forward manner rather than through per-scene optimization. For instance, GPS-Gaussian~\cite{zheng2024gps} performs epipolar rectification and disparity estimation using input image pairs but relies on rectified stereo images and ground-truth depth maps. Spatter Image~\cite{szymanowicz2024splatter} offers a single-view 3D reconstruction approach, primarily focusing on single-object. These methods are often constrained by inefficiencies, limited to object reconstruction, and dependent on specific input formats such as image pairs or single views. In this paper, we extend 3D Gaussian Splatting into visual pre-training tasks, overcoming limitations related to the number of views and the necessity of depth maps by presetting fixed-position 3D Gaussian anchors in 3D space,  marking a novel application of 3D-GS.

\begin{figure*}[ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/cvpr-model-0.pdf}
  \caption{The architecture of proposed GaussianPretrain. Given multi-view images, we first get valid mask patches under MAE technology and LiDAR depth supervision. By constructing 3D voxel features with LSS in these patches, we learn the Gassuain information which is Conceptualizing 3D Gaussian anchors as volumetric LiDAR points. Finally, the predicted attributes of Gaussian parameters are decoded for the downstream vision task. }
  \label{fig:framework}
\end{figure*}

==> sec/2.1_preliminary_methods.tex <==
\section{Preliminary}
\label{sec:formatting}

\subsection{3D Gaussian Splatting.}
3D Gaussian Splatting~\cite{kerbl20233d} demonstrates strong capabilities in scene representation, editing, and novel view synthesis due to its efficient rasterization design and explicit representation. Generally, scenes are represented by a set of Gaussians which are typically initialized from point clouds derived from reconstruction methods or LiDAR data. Each Gaussian is assigned with learnable attributes of \textit{orientation, color, position, scale}, and \textit{opacity}. During rendering, these 3D Gaussians are projected onto the 2D image plane using differentiable rasterization. For scene representation tasks, the Gaussian attributes are iteratively optimized by supervising the rendered output with ground truth images.

For a Gaussian point in the 3D space, it is defined as
\begin{equation}
G(\mathbf{x}) = e^{-\frac{1}{2}(\mathbf{x} - \boldsymbol{\mu})^\top \boldsymbol{\Sigma}^{-1} (\mathbf{x} - \boldsymbol{\mu})}
\end{equation}
with $\mu$ and $\Sigma$ referring to the Gaussian mean center and the 3D covariance matrix. Projected into 2D, we have the 2D covariance matrix $\Sigma' = J W \Sigma W^T J^T$, where the viewing transformation is represented by 
$W$, and the Jacobian matrix $J$ corresponds to the linear approximation of the transformation. Finally, the pixel color is rendered from N ordered Gaussians with the blending equation
\begin{equation}
\label{reder_rgb}
{C}(p) = \sum_{i=1}^{N} c_i \alpha_i \tau
\end{equation}
where $c_i$ is the Gaussian color represented with spherical harmonics and $\alpha_i$ is the opacity related influence of this Gaussian to the current pixel. $\tau = \prod_{j=1}^{i-1} (1 - \alpha_j)$ i is the transmittance.

\section{Method}
The pipeline of our GaussianPretrain is illustrated in the Figure.\ref{fig:framework}. A simple, innovative, and efficient framework for vision pre-training using 3D-GS representation. 
Given $N$ input images $\{{\textbf{I}}^{i}\}_{i=1}^N$, with corresponding projection matrices $\{\textit{\textbf{{P}}}_i \}_{i=1}^N$, $\textit{\textbf{{P}}}_i \in \mathbb{R}^{3 \times 4}$, computed from the intrinsic and extrinsic matrices of cameras.
Our goal is to predict the attributes, including \textit{RGB}, \textit{Depth}, and \textit{occupancy} of $\mathbf{G}_i \in \mathbb{R}^{K}$ by Gaussian parameters $\{ ({\mu}_j, \alpha_j, {\Sigma}_j, {c}_j ) \}_{j=1}^{K}$ for each scene, where ${\mu}_j$, $\alpha_j$, ${\Sigma}_j$ and ${c}_j$ are the 3D Gaussian's position, opacity, covariance, and color information, and $K$ denote the max number of Gaussian points. 
In this section, we first review the process of converting multi-view images into 3D voxel space in ~\Cref{sec:voxel_encoder}. We then detail the generation of valid masked patches under MAE strategy and Depth guidance in ~\Cref{sec:mask_generator}. Finally, the details of GaussianPretrain losses will be presented in ~\Cref{sec:gaussian_decoder}.

\subsection{Voxel Encoder}
\label{sec:voxel_encoder}
{
In most perception tasks, view transformer is typically used to generate Bird’s Eye View (BEV) features, which is then utilized in subsequent tasks. 
% Our method is versatile and can be applied to a wide range of 3D perception tasks. 
In our baseline model, UVTR~\cite{li2022unifying}, we employ the lift-splat-shoot (LSS)\cite{philion2020lift} and extend the channel dimension to incorporate a height dimension, producing 3D voxel features $V\in R^{C \times Z\times H\times W}$, where $C$, $H$, $W$, and $Z$ represent the channel number, dimensions along the $x$, $y$, and $z$ axes, respectively.
}


\subsection{\textbf{Ray-based Depth Guidance Mask Generator}}
\label{sec:mask_generator}
% Given the multi-view images \textit{I}, we randomly drop some patches from these images and replace traditional convolutions in image backbone with sparse convolutions as in SparK, enabling it to handle masked images, similar to MAE in Transformers style. By using this approach, we can guide the model to learn the global context of the image, thereby enhancing the model performance and generalization capability. Subsequently, we employ lift-split-shoot (LSS) as the image-to-bev transform module to construct 3D volume V ∈ RC×Z×H×W from multi-view image features, where C, W, H, Z represent the channel number, the number of x/y/z dimensions in the 3D space respectively.
For computational efficiency concerns, we only focus on learning the Gaussian information from a limited number of \textit{valid masked patches} within the multi-view images, adopting the MAE~\cite{he2022masked} strategy of random patch masking. Furthermore, sparse convolution is employed to replace traditional convolutions for the image backbone, implemented via SparK\cite{tian2023designing}, resulting in $\{{\textbf{M}}\}_{i=1}^m$, where $m$ denote the maximum number of masked patch. This approach enables the model's ability to learn global contextual information, improving the performance and generalization capabilities.



%In autonomous driving, the background (e.g., sky) is not crucial for 3D perception tasks. 
Additionally, we double-check the mask region by verifying the presence of LiDAR points within a certain depth range. For instance, if a set of points project into the masked patch $M_i$ in the images and their depth falls within the range of [a, b], the mask region $M'_i$ is marked as valid. The process is outlined as follows:
\begin{equation}
{M'}_{i=1}^n = 
\begin{cases}
valid,  \text{if } Proj(\text{\textit{{Set}(\textit{pc})}}) \in \{[a, b], M\} \\
not valid,\text{othervise}
\end{cases}
\end{equation} 
where n $\leq$ m. This strategy also ensures that our model concentrates on the foreground, avoiding unnecessary attention to irrelevant background elements like the sky.

Consider the image pixel denoted by $\mathbf{u}=(u_1, u_2, 1)$ which corresponds to a ray $R$ that extends from the camera into 3D space. Along this ray, we sample $D$ ray points $\{p_{j}=\mathbf{u} d_{j}|j=1,...D,\  d_{j}<d_{j+1}\}$. Each sampled ray point $p$ in the valid mask region ${M'}_{i=1}^n$ can be immediately unprojected from camera space to 3D space using the projection matrix $\textit{\textbf{{P}}}_i$, summary as $\mathcal{G}_p^{M'}(\cdot)$. %Finally, we take these selected valid points as Gaussian anchors for the following process.
%as the $x$ center coordinate of the Gaussian anchor.
%
% \begin{equation}
%     x=\prod\nolimits^{-1}_{P} (p)
% \end{equation} 

\subsection{\textbf{Gaussian Parameters Decoder}}
\label{sec:gaussian_decoder}
% xxx Gaussian decoder如何运作的
% Previous works employed NeRF for implicit scene reconstruction, only learning partial geometric information from depth. To address this issue, we explicitly reconstruct 3D scenes based on 3D Gaussian Splatting, introducing 3D anchor Gaussians. These not only synthesize RGB images and depth maps but also occupancy probabilities, allowing for more effective capture of high-quality, fine-grained geometric details. 

% 提出之前方法的问题
%Previous pre-training works employed NeRF~\cite{mildenhall2021nerf} for implicit scene reconstruction, primarily focusing on geometric information derived from depth data, leading to an incomplete understanding of the scene. To address this limitation, we introduce a novel approach that explicitly reconstructs 3D scenes using 3D Gaussian Splatting.
As shown in \Cref{fig:framework}, by conceptualizing $\mathcal{G}_p^{M'} $  as 3D Gaussian anchors, 
% we simultaneously synthesize RGB images, depth maps, and occupancy probabilities. 
this unified representation enables the efficient capture of high-quality, fine-grained details, providing a more comprehensive understanding of the scene.

%
% Each 3D  Gaussian anchor is characterized by attributes 
% $\mathcal{G}=\{ x \in \mathbb{R}^{3} ,c\in \mathbb{R}^{3} ,r\in \mathbb{R}^{4},s\in \mathbb{R}^{3} ,\alpha \in \mathbb{R}^{1} \}$
% , representing the 3D position, color, rotation, scaling, and opacity, respectively. In this section, we introduce how to formulate 3D Gaussian anchor in 3D space. Specifically, the proposed Gaussian maps $G$ are defined as
Specially, each 3D  Gaussian anchor is characterized by attributes 
$\mathcal{G}=\{ x \in \mathbb{R}^{3} ,c\in \mathbb{R}^{3} ,r\in \mathbb{R}^{4},s\in \mathbb{R}^{3} ,\alpha \in \mathbb{R}^{1} \}$
and the proposed Gaussian maps $G$ are defined as:
\begin{equation}
G\left( x\right)  =\{ \mathcal{M}_{c} (x),\mathcal{M}_{r} (x),\mathcal{M}_{s} (x),\mathcal{M}_{\alpha } (x)\} 
\end{equation}
%
where $x$ is the position of a Gaussian anchor in 3D space, $\mathcal{M}_{c}$, $\mathcal{M}_{r}$, $\mathcal{M}_{s}$, $\mathcal{M}_{\alpha }$ represents Gaussian parameters maps of color, rotation, scaling and opacity, respectively.

% In more detail, let $\mathbf{u} =(u_{1},u_{2},1)$ denote one of the image pixels. This corresponds to a $R$ ray, then we sample $D$ ray points $\{p_{j}=\mathbf{u} d_{j}|j=1,...D,\  d_{j}<d_{j+1}\}$ in camera space, where $p_{j}$ corresponds to the depth along the $R$ ray. Each ray point $p$ can be immediately unprojected from camera space to 3D space using the projection matrix $P\in \mathbb{R}^{3\times 4} $ structured with camera parameters $K$, as the $\x$ center coordinate of the Gaussian anchor.

%
Due to the overlapping areas in the multi-view images, the pixel-by-pixel prediction of Gaussian parameters % similar to the splatter image 
may lead to ambiguity due to overlapping splats. In contrast, we argue that predicting Gaussian parameters directly from 3D voxel features is a better choice. Given voxel features $V$ and center coordinate $x$ , we employ trilinear interpolation to sample the corresponding feature $f(x)$ as follows:
%
\begin{equation}
f(x)=TriInter(V,x)
\end{equation}
% The prediction heads, each composed of MLP layers, are adapted to Gaussian features for specific Gaussian parameter map regression. 
The Gaussian parameter maps are generated by prediction heads,  defined as $h=MLP(\cdot)$, which consist of multiple MLP layers. Each prediction head is specifically designed to regress a particular parameter based on the sampled feature $f(x)$. For the  parameter of color and opacity, we employed the sigmoid function for a range of [0,1] as follows:
\begin{align}
    \mathcal{M}_{c} (x)=Sigmoid(h_{c}(f(x)) \\
    \vspace{1em}
    \mathcal{M}_{\alpha} (x)=Sigmoid(h_{\alpha}(f(x))
\end{align}
%
Where $h_{c}$, $h_{\alpha}$ denote the head of color and opacity. 

Before being used to formulate Gaussian representations, the rotation map should be normalized since it represents a quaternion to ensure unit magnitude while the scaling map needs activations to satisfy their range as follows:
%
\begin{align}
    \mathcal{M}_{r} (x)=Norm(h_{r}(f(x))\\
    \vspace{1em}
    \mathcal{M}_{s} (x)=Softplus(h_{s}(f(x)) 
\end{align}
%
Where $h_{r}$, $h_{s}$ represents the rotation head and scale head.
%
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/cvpr-gaussian-1.pdf}
  \caption{
  %
  \textbf{Process of generating valid mask patches. } 
 }
  \label{fig:motivation}
\end{figure}


\input{tables/OD_matrixs}


% \begin{table*}[!t]
%     \caption{Comparisons of different models pre-trained with our GaussianPretrain in the HD map construction task}
%     \centering
%     \resizebox{\textwidth}{!}{%     % columnwidth: 代表扩宽为当前列， textwidth: 代表扩宽为当前文章
%         \begin{tabular}{l|c|c|c|c|ccc}
%         \toprule
%          \textbf{\# Model} & 
%          \textbf{Backbone} & 
%          \textbf{Pretrain} & 
%          \textbf{Epochs} & 
%          \textbf{mAP$\uparrow$} &
%          \textbf{AP$_{ped}\uparrow$} &
%          \textbf{AP$_{divider}\uparrow$} &
%          \textbf{AP$_{boundary}\uparrow$} 
%          \\
%         \bottomrule
%             HDMapNet & EfficientNet-B0 & ImageNet  & 30 & 23.0 &14.4 &21.7 &33.0  \\
%             VectorMapNet & ResNet50 & ImageNet  & 110 & 40.9 &36.1 &47.3 &39.3  \\
%             \hline
%             \multirow{2}{*}{MapTR~\cite{liao2022maptr}} & ResNet50 & ImageNet  & 24 & 49.9 &52.0 &45.3 &52.4  \\
%                   & ResNet50 & GaussianPretrain  & 24 & 51.8 &54.9 &45.8 &54.9  \\
%         \bottomrule
%         \end{tabular}
%     }
%     \label{tab:Comparsion-HDMap}
% \end{table*}

\input{tables/HD-Map_matrixs}

\input{tables/OCC_matrixs}

\subsection{\textbf{Supervise with Differentiable Rendering}}
% 介绍用到的loss
% To achieve unsupervised learning without any labels, we Unlike Unipad supervised model in 2D plane with Nerf, we use Differentiable Rendering supervised model in 2D plane and 3D space, 加强了模型对场景的理解。Specifically, 在我们预测出Gaussian anchor parameter后，we employ 3D Gaussian splatting to syntheize color maps and depth maps. 我们可以采用类似Unipad的方法在2d plane上监督模型。此外，由于我们将Gaussian anchor 看作是体积化的lidar，我们可以完成occupancy reconstruction 监督，在3D space 提高模型对场景的理解。
To enable unsupervised learning without relying on labels, we deviate from the  NeRF~\cite{mildenhall2021nerf} base method, UniPAD~\cite{yang2024unipad}, instead with \textit{Differentiable Rendering} which operates in both the 2D and 3D space to enhance the model's understanding of the scene. Specifically, we employ 3D Gaussian splatting to synthesize color maps, depth maps, and opacity after predicting the Gaussian anchor parameters. 
%\textcolor{red}{Similar to the approach used in UniPAd, we can supervise the model in the 2D plane.}
%Additionally, since we treat the Gaussian anchor as volumetric representation similar to LiDAR and learned opacity information, we can perform occupancy reconstruction supervision in the 3D space, further improving the model's scene comprehension.

\noindent \textbf{Rendering RGB.}
Since we do not need to render images of arbitrary perspectives, we directly predict fixed view \textit{RGB} instead of \textit{Spherical Harmonics {(SH)}} coefficients.
After predicting the parameters of the Gaussian anchor, we decode the color information with the  \Cref{reder_rgb} from 3D Gaussian splatting, specifically to render the RGB values $\hat{C} $.

\noindent \textbf{Rendering Depth.}
For each-pixel z-depth, $\hat{D}$ are rendered with discrete volume rendering approximation similar to RGB, which is decoded from the 3D-GS parameters.
\begin{equation}
\hat{D} =\sum_{i=1}^k d_{i}\alpha_{i} \prod^{i-1}_{j=1} (1-\alpha_{j} )
\end{equation}
%
where k is the number of sampling points along the ray, $d_{i}$ is the $i^{th}$ Gaussian anchor $z$-depth coordinate in view space.
%

\noindent \textbf{Reconstructing Occupancy}
% The opacity attribute of 3D-GS point is inherent to vision perception, especially occupancy task.
% Unlike GaussianFormer\cite{huang2024gaussianformer}, we treat the opacity as occupancy instead of semantic logits to predict whether or not the 3D space is occupied.  We argue that this is reasonable: when a Gaussian anchor exists, the transparency is zero, meaning the voxel at the Gaussian anchor's location $x$ is considered occupied. We further define that the 3D voxel containing the Gaussian anchor, this voxel is treated as an occupancy target $\hat{O}$.
The opacity attribute of 3D-GS point is inherent to vision perception, particularly for occupancy prediction tasks.
Unlike GaussianFormer\cite{huang2024gaussianformer}, which uses opacity for semantic logits, we directly interpret opacity as an indicator of occupancy. This interpretation is based on the observation that a Gaussian anchor with zero transparency signifies the presence of an occupied voxel at its location $x$.  More formally, we define the 3D voxel containing a Gaussian anchor as an occupied voxel, denoted by the occupancy target $\hat{O}$. This direct mapping of opacity to occupancy provides a natural and effective way to leverage 3D Gaussian Splatting for occupancy prediction.
%
\subsection{\textbf{Loss Function}}

% Unlike tasks focused on novel view synthesis, which use dense supervision to enhance rendered image quality, our objective is to pre-train the backbone rather than to produce high-quality images. Following UniPAD~\cite{yang2024unipad}, we use a depth-aware sampling strategy that projects the lidar point cloud onto multi-view images, selects pixels with depths below a certain threshold, and then randomly chooses $N$ pixels from this set for supervision. In addition to reducing computational complexity, this strategy also ensures that our model concentrates on the foreground, avoiding unnecessary attention to irrelevant background elements like the sky.

In summary, the overall pre-training loss function consists of the color loss, depth loss and occupancy loss:
%
\begin{equation}
\begin{aligned}
\resizebox{\linewidth}{!}{$
\begin{gathered}L=\frac{\lambda_{RGB} }{N} \sum^{N}_{i=1} \left| C_{i}-\hat{C}_{i} \right|  +\frac{\lambda_{Depth} }{N} \sum^{N}_{i=1} \left| D_{i}-\hat{D}_{i} \right|  \\ +\frac{\lambda_{Occupacy} }{M} \sum^{M}_{i=1} \left| O_{i}-\hat{O}_{i} \right|  \end{gathered} 
$}.
\end{aligned}
\end{equation}
%
where $C_{i}$, ${D}_{i}$ and $O_{i}$  are the lable color, depth and occupancy, respectively. $N$ is the count of Gaussian anchor.

==> tables/diff_backone.tex <==
\begin{table}[t]
  \centering
  \setlength{\tabcolsep}{1.2mm}
  \scalebox{0.8}{
  \begin{tabular}{{l|l|l|cc}}
    \toprule[1.5pt]
    Methods  & \multicolumn{1}{c|}{ \multirow{1}{*}{Encoder}} & \multicolumn{1}{c|}{ \multirow{1}{*}{Pre-train}} & mAP (\%) & NDS (\%) \\
    \midrule
    \multicolumn{1}{c|}{ \multirow{6}{*}{\makecell[l]{BEV-\\Former} \cite{li2022bevformer}}} & \multicolumn{1}{c|}{ \multirow{2}{*}{RN50 \cite{ResNet}}} & ImageNet \cite{imagenet_cvpr09} & 25.2 & 35.4 \\
     & & GaussianPretrain & \cellcolor{lightgray}\bf 29.0 & \cellcolor{lightgray}\bf 38.8 \\
     \cmidrule{2-5}
     & \multicolumn{1}{c|}{ \multirow{2}{*}{RN101 \cite{ResNet}}} & ImageNet \cite{imagenet_cvpr09} & 37.7 & 47.7  \\
     &  & GaussianPretrain & \cellcolor{lightgray}\bf 42.6 & \cellcolor{lightgray}\bf 51.8 \\
     \cmidrule{2-5}
     & \multicolumn{1}{c|}{ \multirow{2}{*}{ConverNext-S}} & ImageNet \cite{lin2014coco} & 41.5 & 51.2 \\
     & & GaussianPretrain & \cellcolor{lightgray}\bf 47.6  & \cellcolor{lightgray}\bf 56.4 \\
    \bottomrule[1.5pt]
  \end{tabular}
  }
  \vspace{-0.1in}
  \caption{\textcolor{red}{TODO.}\textbf{
  Detection performance} of BEVFormer with and without GaussianPretrain pre-training under various backbones and initializations.
  }
  \label{tab:detection}
\end{table}

